LoCa: Logit Calibration for Knowledge Distillation

Knowledge Distillation (KD), aiming to train a better student model by mimicking the teacher model, plays an important role in model compression. One typical way is to align the output logits. However, we find a common issue named mis-instruction, that the student would be misled when the predictions based on teacher logits do not follow the labels. Meanwhile, there is other useful dark knowledge in the logits such as the class discriminability, which is vital for distillation. In this paper, we propose a simple yet effective Logit Calibration (LoCa) method, which calibrates the logits from the teacher model based on the ground-truth labels. The key insight is to correct the prediction (to address the mis-instruction issue) and maintain useful dark knowledge simultaneously. Our proposed LoCa does not require any additional parameters. Empirical results on image classification and text generation tasks demonstrate that LoCa can effectively improve the performance of baselines.

==> graph_table/table_analysis_alpha.tex <==

\begin{table}[!t]
\centering
\caption{Sensitivity of  LoCa hyperparameter $\alpha$ from \textbf{ResNet32} to \textbf{ResNet18}. Top-1 and Top-5 accuracy (\%) are shown. The baseline represents the vanilla KD approach.}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{\textbf{Metric}} & \multirow{2}{*}{\textbf{Baseline}} & \multicolumn{6}{c}{\textbf{The value of $\alpha$ in LoCa}} \\
\cmidrule{3-9}
& & 
\textbf{0.950} & \textbf{0.980} & \textbf{0.985}  & \textbf{0.990} & \textbf{0.995} & \textbf{0.999} \\
\midrule
Top-1  & 71.03 & 71.08 & 71.21 & 71.24 & 71.16 & \textbf{71.36} & 71.12  \\
Top-5  & 90.05 & 90.06 & 90.13 & 90.12 & \textbf{90.24} & 90.16 & 90.08 \\
\bottomrule
\end{tabular}
}

\label{tab:ablation_alpha}
\end{table}


==> graph_table/table_dataset_CV.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Dataset split for CIFAR-100 and ImageNet.}}
\begin{small}
\begin{tabular}{ccccc}
\toprule
\textbf{Dataset Name} & \textbf{Usage} & \textbf{Samples} \\
\midrule
\multirow{2}{*}{CIFAR-100} & Train & 50,000 \\
\cmidrule{2-3}
& Valid & 10,000 \\
\midrule
\multirow{2}{*}{ImageNet} & Train & 1,280,000 \\
\cmidrule{2-3}
& Valid & 50,000 \\
\bottomrule
\end{tabular}

\label{tab:dataset_cifar_imagenet}
\end{small}
\end{table}


==> graph_table/table_result_LLM.tex <==

\begin{table}[!h]
\centering
\begin{tabular}{lcccccc}
\toprule
\multirow{3}{*}{\bf Method}  
      & \multicolumn{3}{c}{\bf LLaMA 6.7B $\rightarrow$ TinyLLaMA 1.1B} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \colorbox{yellow}{Dolly} & S-NI & UnNI \\
 & (500) & (1694) & (10000) \\
\midrule
Teacher           & 26.73$\pm$0.65                                            & 32.75$\pm$0.24                                           & 34.61$\pm$0.08                                             \\  
SFT  & 22.05$\pm$0.38                                            & 27.79$\pm$0.20                                           & 25.96$\pm$0.13                                             \\
KD        & 22.24$\pm$0.38                                            & 28.07$\pm$0.41                                           & 26.93$\pm$0.09 \\
\rowcolor{gg}{LoCa~(Ours)} & \textbf{ 22.54$\pm$0.34 }                                   & \textbf{28.24$\pm$0.28}                                  & \textbf{27.12$\pm$0.13}                                    \\ \bottomrule
\end{tabular}
% }
\caption{The results of Rouge-L scores under LLaMA 6.7B to TinyLLaMA 1.1B .
Our proposed LoCa outperforms baseline without any extra parameters.}
\label{main_res_text}
\end{table}

